System Architecture and Communication Infrastructure for the RoboVaaS project

Current advancements in waterborne autonomous systems, together with the development of cloud-based service-oriented architectures and the recent availability of low-cost underwater acoustic modems and long-range above water wireless devices, enabled the development of new applications to support ships and port activities. Unmanned Surface Vehicle (USV) can, for instance, be used to perform bathymetry and environmental data collection tasks to ensure under-keel clearance and to monitor the quality of the water. Similarly, Remotely Operated Vehicles (ROVs) can be deployed to inspect ship hulls and typical port infrastructure elements, such as quay and sheet pilling walls. In this paper we present the complete system deployed for the small-scale demonstrations of the Robotic Vessels as-a-Service (RoboVaaS) project, which introduces an on-demand service-based cloud system that dispatches Unmanned Vehicles (UVs) capable of performing the required service either autonomously or piloted. These vessels are able to interact with sensors deployed in the port and with the shore station through an integrated underwater and above water network. The developed system has been validated through sea trials and showcased through an underwater sensor data collection service. The results of the test presented in this paper provide a proof-of-concept of the system design and indicate its technical feasibility. It also shows the need for further developments for a mature technology allowing on-demand robotic maritime assistance services in real operational scenarios.

==> figures/smp_plots/pdr_buoy_to_seaml.plot.tex <==
\newcommand{\data}{data/pdr/buoy_to_seaml.dat}
\input{pdr.plot.inc}

==> figures/smp_plots/pdr_seaml_to_buoy.plot.tex <==
\newcommand{\data}{data/pdr/seaml_to_buoy.dat}
\input{pdr.plot.inc}

==> figures/smp_plots/psd_noisefree.plot.tex <==
\newcommand{\data}{data/psd/noisefree.dat}
\input{psd.plot.inc}

==> figures/smp_plots/psd_noisefree_pkt.plot.tex <==
\newcommand{\data}{data/psd/noisefree_pkt.dat}
\input{psd.plot.inc}

==> figures/smp_plots/psd_seaml.plot.tex <==
\newcommand{\data}{data/psd/seaml.dat}
\input{psd.plot.inc}

==> figures/smp_plots/psd_seaml_pkt.plot.tex <==
\newcommand{\data}{data/psd/seaml_pkt.dat}
\input{psd.plot.inc}

==> figures/smp_plots/setup/color_setup.tex <==
\pgfplotsset{signal/.style = {%
  cycle list name = tuhh cycle list no marks,
  solid,
  thick,
}}


\pgfplotsset{ybar error/.style={%
%   error y both,
%   only marks,
%   mark = *,
%   mark size = 1pt,
% %   fill = uzl_turquoise_4,
%   draw = uzl_gray_4,
  %       point meta = y,
%     every node near coord/.style={inner ysep=5pt},
%error y both,
  error bars/.cd,
    y dir = both,
    y explicit,
    error mark = |,
    error mark options = {mark size = 1pt},
    error bar style = {solid, line width = 0.5pt},
}}


\pgfplotsset{colormap={colormap_freq}%
%{color=(uzl_white) color=(uzl_turquoise_3) color=(uzl_yellow_2) color=(uzl_red_2) color=(uzl_black)}}
{color=(tuhh_white) color=(tuhh_darkturquoise) color=(tuhh_yellow) color=(tuhh_darkred) color=(tuhh_black)}}
 %color=(uzl_mediumblue_2)

%\pgfplotsset{colormap={colormap_load}%
%{color(0cm)=(tuhh_white) color(1cm)=(tuhh_lightblue) color(4cm)=(tuhh_magenta)}}



\pgfplotsset{%
  stat/.style = {%
    fill opacity = 0.8,
    tuhh_turquoise,
    line width=0.0pt,
    solid,
  },
  stat min/.style = {%
    draw = none,
    fill = none,
    no markers
  },
  stat inner quartiles/.style = {%
    stat,
    draw = none,
    fill = tuhh_turquoise,
  },
  stat outer quartiles/.style = {%
    stat,
    fill = tuhh_turquoise!50!tuhh_white,
  },
  stat median/.style = {%
    %stat,
    fill = none,
    draw = tuhh_blue,
    line width=1.0pt,
    %every mark/.append style = {fill=tuhh_darkred,draw=none,fill opacity=1},
    %mark=*, mark size=2pt,
  }
}


==> figures/smp_plots/setup/pgfplots_setup.tex <==
% ColorBrewer
% draw: 8-class Dark2
% fill: 8-class Set2
% fill: 8-class Pastel2
\definecolor{draw-1}{RGB}{27,158,119}
%\definecolor{fill-1}{RGB}{102,194,165}
\definecolor{fill-1}{RGB}{179,226,205}

\definecolor{draw-2}{RGB}{217,95,2}
%\definecolor{fill-2}{RGB}{252,141,98}
\definecolor{fill-2}{RGB}{253,205,172}

\definecolor{draw-3}{RGB}{117,112,179}
%\definecolor{fill-3}{RGB}{141,160,203}
\definecolor{fill-3}{RGB}{203,213,232}

\definecolor{draw-4}{RGB}{231,41,138}
%\definecolor{fill-4}{RGB}{231,138,195}
\definecolor{fill-4}{RGB}{244,202,228}

\definecolor{draw-5}{RGB}{102,166,30}
%\definecolor{fill-5}{RGB}{166,216,84}
\definecolor{fill-5}{RGB}{230,245,201}

\definecolor{draw-6}{RGB}{230,171,2}
%\definecolor{fill-6}{RGB}{255,217,47}
\definecolor{fill-6}{RGB}{255,242,174}

\definecolor{draw-7}{RGB}{166,118,29}
%\definecolor{fill-7}{RGB}{229,196,148}
\definecolor{fill-7}{RGB}{241,226,204}

\definecolor{draw-8}{RGB}{102,102,102}
%\definecolor{fill-8}{RGB}{179,179,179}
\definecolor{fill-8}{RGB}{204,204,204}


%% shaded colors
% PINK
\definecolor{pink-8-1}{RGB}{247,244,249}
\definecolor{pink-8-2}{RGB}{231,225,239}
\definecolor{pink-8-3}{RGB}{212,185,218}
\definecolor{pink-8-4}{RGB}{201,148,199}
\definecolor{pink-8-5}{RGB}{223,101,176}
\definecolor{pink-8-6}{RGB}{231,41,138}
\definecolor{pink-8-7}{RGB}{206,18,86}
\definecolor{pink-8-8}{RGB}{145,0,63}

% GREEN
\definecolor{green-8-1}{RGB}{255,255,229}
\definecolor{green-8-2}{RGB}{247,252,185}
\definecolor{green-8-3}{RGB}{217,240,163}
\definecolor{green-8-5}{RGB}{120,198,121}
\definecolor{green-8-4}{RGB}{173,221,142}
\definecolor{green-8-6}{RGB}{65,171,93}
\definecolor{green-8-7}{RGB}{35,132,67}
\definecolor{green-8-8}{RGB}{0,90,50}

% BLUE
\definecolor{blue-8-1}{RGB}{247,251,255}
\definecolor{blue-8-2}{RGB}{222,235,247}
\definecolor{blue-8-3}{RGB}{198,219,239}
\definecolor{blue-8-4}{RGB}{158,202,225}
\definecolor{blue-8-5}{RGB}{107,174,214}
\definecolor{blue-8-6}{RGB}{66,146,198}
\definecolor{blue-8-7}{RGB}{33,113,181}
\definecolor{blue-8-8}{RGB}{8,69,148}

% GRAY
\definecolor{gray-8-1}{gray}{0.95}
\definecolor{gray-8-2}{gray}{0.90}
\definecolor{gray-8-3}{gray}{0.85}
\definecolor{gray-8-4}{gray}{0.75}
\definecolor{gray-8-5}{gray}{0.60}
\definecolor{gray-8-6}{gray}{0.40}
\definecolor{gray-8-7}{gray}{0.20}
\definecolor{gray-8-8}{gray}{0.05}

%%%


\pgfplotscreateplotcyclelist{tuhh cycle list}{%
  draw-1,every mark/.append style={fill=fill-1},mark=*,mark size=1.4pt\\%
  draw-2,every mark/.append style={fill=fill-2},mark=square*,mark size=1.2pt\\%
  draw-3,every mark/.append style={fill=fill-3},mark=diamond*,mark size=1.8pt\\%
  draw-4,every mark/.append style={fill=fill-4},mark=triangle*,mark size=1.8pt\\%
  draw-5,every mark/.append style={fill=fill-5},mark=pentagon*,mark size=1.5pt\\%
  %draw-6,every mark/.append style={fill=fill-6},mark=pentagon*,mark size=1.5pt\\%
  %draw-7,every mark/.append style={fill=fill-7},mark=pentagon*,mark size=1.5pt\\%
  %draw-8,every mark/.append style={fill=fill-8},mark=pentagon*,mark size=1.5pt\\%
}

\pgfplotscreateplotcyclelist{tuhh cycle list no marks}{%
  draw-1,mark=none\\%
  draw-2,mark=none\\%
  draw-3,mark=none\\%
  draw-4,mark=none\\%
  draw-5,mark=none\\%
  draw-6,mark=none\\%
  draw-7,mark=none\\%
  draw-8,mark=none\\%
}


\pgfdeclarepatternformonly{bar north east lines}{\pgfqpoint{-1pt}{-1pt}}{\pgfqpoint{4pt}{4pt}}{\pgfqpoint{3pt}{3pt}}%
{
  \pgfsetlinewidth{0.8pt}
  \pgfpathmoveto{\pgfqpoint{0pt}{0pt}}
  \pgfpathlineto{\pgfqpoint{3.1pt}{3.1pt}}
  \pgfusepath{stroke}
}

\pgfdeclarepatternformonly{bar north west lines}{\pgfqpoint{-1pt}{-1pt}}{\pgfqpoint{4pt}{4pt}}{\pgfqpoint{3pt}{3pt}}%
{
  \pgfsetlinewidth{0.8pt}
  \pgfpathmoveto{\pgfqpoint{0pt}{3.1pt}}
  \pgfpathlineto{\pgfqpoint{3.1pt}{0pt}}
  \pgfusepath{stroke}
}

% \pgfdeclarepatternformonly{bar vertical lines}{\pgfqpoint{-1pt}{-1pt}}{\pgfqpoint{2pt}{3pt}}{\pgfqpoint{1pt}{2pt}}%
% {
%   \pgfsetlinewidth{0.5pt}
%   \pgfpathmoveto{\pgfqpoint{.5pt}{0pt}}
%   \pgfpathlineto{\pgfqpoint{.5pt}{2.1pt}}
%   \pgfusepath{stroke}
% }

\pgfdeclarepatternformonly{bar checker}{\pgfqpoint{-1pt}{-1pt}}{\pgfqpoint{2pt}{2pt}}{\pgfqpoint{2pt}{2pt}}%
{
  %\pgfsetlinewidth{0.8pt}
  \pgfpathmoveto{\pgfqpoint{1.0pt}{0.0pt}}
  \pgfpathlineto{\pgfqpoint{2.0pt}{1.0pt}}
  \pgfpathlineto{\pgfqpoint{1.0pt}{2.0pt}}
  \pgfpathlineto{\pgfqpoint{0.0pt}{1.0pt}}
  \pgfpathclose%
  \pgfsetnonzerorule
  \pgfusepath{fill}
}

\pgfdeclarepatternformonly{bar crosshatch}{\pgfqpoint{-1pt}{-1pt}}{\pgfqpoint{4pt}{4pt}}{\pgfqpoint{3pt}{3pt}}%
{
  \pgfsetlinewidth{0.8pt}
  \pgfpathmoveto{\pgfqpoint{3.1pt}{0pt}}
  \pgfpathlineto{\pgfqpoint{0pt}{3.1pt}}
  \pgfpathmoveto{\pgfqpoint{0pt}{0pt}}
  \pgfpathlineto{\pgfqpoint{3.1pt}{3.1pt}}
  \pgfusepath{stroke}
}

\pgfdeclarepatternformonly{bar grid}{\pgfqpoint{-1pt}{-1pt}}{\pgfqpoint{3pt}{3pt}}{\pgfqpoint{2pt}{2pt}}%
{
  \pgfsetlinewidth{0.4pt}
  \pgfpathmoveto{\pgfqpoint{0.0pt}{0.8pt}}
  \pgfpathlineto{\pgfqpoint{2.1pt}{0.8pt}}
  \pgfpathmoveto{\pgfqpoint{1.0pt}{0.0pt}}
  \pgfpathlineto{\pgfqpoint{1.0pt}{2.1pt}}
  \pgfusepath{stroke}
}

\pgfdeclarepatternformonly{bar horizontal zigzag}{\pgfqpoint{-1pt}{-1pt}}{\pgfqpoint{3pt}{3pt}}{\pgfqpoint{2pt}{2pt}}%
{
  \pgfsetlinewidth{0.4pt}
  \pgfpathmoveto{\pgfqpoint{0.0pt}{0.0pt}}
  \pgfpathlineto{\pgfqpoint{1.0pt}{1.0pt}}
  \pgfpathlineto{\pgfqpoint{2.0pt}{0.0pt}}
  \pgfusepath{stroke}
}

\pgfdeclarepatternformonly{bar dots}{\pgfqpoint{-1pt}{-1pt}}{\pgfqpoint{2pt}{2pt}}{\pgfqpoint{2pt}{2pt}}%
{
  \pgfpathcircle{\pgfqpoint{0pt}{0pt}}{.5pt}
  \pgfpathcircle{\pgfqpoint{1pt}{1pt}}{.5pt}
  \pgfusepath{fill}
}


\pgfplotsset{%
  /pgfplots/bar cycle list/.style = {/pgfplots/cycle list = {%
    {draw-1, fill = fill-1, mark = none},%
    %
    {draw-2, fill = fill-2, mark = none, pattern color = draw-2,
      postaction = {pattern = bar north east lines, pattern color = draw-2, opacity = 0.5}},%
    %
    {draw-3, fill = fill-3, mark = none, pattern color = draw-3,
      postaction = {pattern = bar checker, pattern color = draw-3, opacity = 0.5}},%
    %
    {draw-4, fill = fill-4, mark = none, pattern color = draw-4,
      postaction = {pattern = bar north west lines, pattern color = draw-4, opacity = 0.5}},%
    %
    {draw-5, fill = fill-5, mark = none, pattern color = draw-5,
      postaction = {pattern = bar dots, pattern color = draw-5, opacity = 0.5}},%
    %
    {draw-6, fill = fill-6, mark = none, pattern color = draw-6,
      postaction = {pattern = bar crosshatch, pattern color = draw-6, opacity = 0.5}},%
  }},
}


\pgfplotsset{%
  /pgfplots/rx cycle list/.style = {
    mark = none,
    ultra thin,
    %draw = transparent,
    /pgfplots/cycle list = {%
    {fill = green-8-7, draw = green-8-8},%
    %
    {fill = green-8-6, draw = green-8-8},%
    %
    {fill = green-8-5, draw = green-8-8},%
    %
    {fill = green-8-4, draw = green-8-8},%
    %
    {fill = green-8-3, draw = green-8-8},%
    %
    {fill = green-8-1, draw = green-8-8},%
    %
    %
    {fill = blue-8-7, draw = blue-8-8},%
    %
    {fill = blue-8-6, draw = blue-8-8},%
    %
    %
    {fill = pink-8-7,  draw = pink-8-8,
      postaction = {pattern = bar north east lines, pattern color = white, opacity = 0.3}},%
    %
    {fill = pink-8-7,  draw = pink-8-8,
      postaction = {pattern = bar north east lines, pattern color = white, opacity = 0.6}},%
    %
    {fill = pink-8-7,  draw = pink-8-8,
      postaction = {pattern = bar north west lines, pattern color = white, opacity = 0.3}},%
    %
    {fill = pink-8-7,  draw = pink-8-8,
      postaction = {pattern = bar north west lines, pattern color = white, opacity = 0.6}},%
  }},
}


\pgfplotsset{%
  /pgfplots/rxstat cycle list/.style = {%
    thin,
    /pgfplots/cycle list = {%
      %{fill = tuhh_orange!80!tuhh_white, draw = tuhh_orange!90!tuhh_white, mark=none},%
      %
      {fill = blue-8-6, draw = blue-8-8, mark=none,
        postaction = {pattern = bar north east lines, pattern color = blue-8-2}},%
      %
      {fill = blue-8-6, draw = blue-8-8, mark=none,
        postaction = {pattern = bar north west lines, pattern color = blue-8-4}},%
      %
      {fill = blue-8-6, draw = blue-8-8, mark=none},%
    },
  },
}

\pgfplotsset{%
  /pgfplots/ping pong cycle list/.style = {%
    /pgfplots/cycle list = {%
      {fill = fill-1, draw = draw-1},%
      {fill = fill-2, draw = draw-2},%
    },
  },
}



\pgfplotsset{no background/.style={
  axis background/.append style={fill=none}
}}

\pgfplotsset{every axis legend/.style={%
  scale only axis,
  % SHAPE and POSITION
  shape   = rectangle,
  fill    = white,
  opacity = 0.8,
  draw    = none,
  anchor  = north east,
  at      = {(0.99,0.99)},
  font    = \scriptsize,
  % CELLS and SPACING
  cells = {anchor = west},% left aligned
  inner xsep = 1pt,
  inner ysep = 1pt,
  nodes = {%
    inner xsep = 2pt,
    inner ysep = 1pt,
    text depth = 0.05em,
  },
  /tikz/every even column/.append style = {column sep = 0.25cm},
}}


% axis style
\pgfplotsset{every axis/.style={%
  axis background/.style = {fill = white},
  try min ticks = 4,
  xlabel near ticks,
  %ylabel near ticks,
  grid = both, tick align=inside, tickpos=left,
  major grid style = {solid, line width=0.6pt, gray-8-6},
  minor grid style = {solid, line width=0.2pt, gray-8-4},
  tick label style = {%
    font = \scriptsize,
    /pgf/number format/1000 sep = \,,
    /pgf/number format/zerofill,
    /pgf/number format/fixed
  },
  x tick label style = {anchor = base, yshift = -1em},
  %x tick label style={},
  %y tick label style={},
  title style = {font = \footnotesize, at = {(rel axis cs:0.5,1.0)}, anchor = base }
}}


\pgfplotsset{tufte grid/.style={%
  axis on top,
  tick style = {draw = none},
  grid = both, %tick align=outside, tickpos=left,
  major  = {%
    solid,
    white
    line width = 0.5pt,
  },
  minor grid style = {%
    dash pattern = on \pgflinewidth off .2pt,
    line width   = 0.2pt,
    white,
  },
  %axis x line* = bottom,
  %axis y line* = none,
}}

\tikzset{legend label/.style = {%
  shape   = rectangle,
  rounded corners = 1pt,
  fill    = white,
  opacity = 1.0,
  fill opacity = 0.8,
  draw    = none,
  anchor  = base,
  font    = \scriptsize,
  inner xsep = 2pt,
  inner ysep = 1pt,
}}

\pgfplotsset{inside ticks/.style={%
  tick align = inside,
  tickpos    = both,
}}

\pgfplotsset{outside ticks/.style={%
  tick align = outside,
  tickpos    = both,
}}

\pgfplotsset{every axis label/.style={%
  font = \footnotesize,
}}


\pgfplotsset{extra right ticks/.style = {%
  extra y tick style = {%
    grid = major,
    major grid style = {%
      solid,
      pink-8-7,
      line width = 0.5pt,
    },
    tick pos = right,
    major tick length = 0pt,
    ticklabel pos = right,
    tick label style = {%
      color = pink-8-7,
      font = \tiny,
      xshift = -2pt
  }}
}}

\pgfplotsset{no x grid/.style = {%
  xmajorgrids = false,
  xtick align = inside,
  xtick style = { draw = none, },
  major tick length = 0pt
}}

\pgfplotsset{no y grid/.style = {%
  ymajorgrids = false,
  ytick align = inside,
  ytick style = { draw = none, },
  major tick length = 0pt
}}

\pgfplotsset{no grid/.style = {%
  grid style = {draw = none}, 
}}


% pins (labels in graphs)
%\tikzset{
%  every pin/.style={fill=uzl_yellow_1,draw=uzl_gray_1,thin,rectangle,rounded corners=2pt,font=\scriptsize,inner sep=1pt,minimum height=9pt},
%  small dot/.style={fill=none,draw=uzl_gray_4,circle,scale=0.4,thick},
%}

% helpers (arrows and labels)
%\tikzstyle{help label}=[anchor=south,font=\scriptsize,very thin,inner sep=1pt,color=uzl_intenseblue_3,fill=tuhh_gray,draw=tuhh_darkgray, rounded corners=1pt]
%\tikzstyle{help arrow}=[->,>=latex',tuhh_darkgray]

%%%%%%%%%%%%%%%%%%%% ERROR PLOT %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\pgfplotsset{error y plus/.style={
  mark = *, mark size=1.4pt,
  error bars/.cd,
  y dir = plus,
  y explicit,
  }%
}

\pgfplotsset{error y both/.style={
  error bars/.cd,
  mark = o, mark size=1.4pt,
  error bars/.cd,
  y dir = both,
  y explicit,
  /pgfplots/.cd
  }%
}

\pgfplotsset{error x plus/.style={
  mark = *, mark size=1.4pt,
  error bars/.cd,
  x dir = plus,
  x explicit,
  /pgfplots/.cd
  }%
}

\pgfplotsset{error xy plus/.style={
  mark = *, mark size=1.4pt,
  x dir = plus,
  x explicit,
  y dir = plus,
  y explicit}%
}



%%%%%%%%%%%%%%%%%%%% GROUPED PLOTS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\tikzset{%
  group splitter/.style = {%
    gray-8-3,
    opacity    = 0.25,
    draw       = gray-8-7,
    line width = 0.3pt,
  },
}

% \pgfplotsset{%
%   draw splitters/.code = {%
%     \drawSplitters{#1}
%   }
% }

\newcommand{\drawSplitters}[1]{%
  \pgfmathint{#1}
  \edef\bins{\pgfmathresult}
  %
  \foreach \i in {1,3,...,\bins}{
    \pgfmathparse{\i*1.0/\bins}
    \edef\ll{\pgfmathresult}
    \pgfmathparse{(\i+1)/\bins}
    \edef\rr{\pgfmathresult}
    \edef\temp{%
      \noexpand%
      \fill[group splitter] (rel axis cs:\ll,0) rectangle (rel axis cs:\rr,1);%
    }
    \temp
    %;
  }
}


\newcommand{\drawVSplitters}[1]{%
  \pgfmathint{#1}
  \edef\bins{\pgfmathresult}
  %
  \foreach \i in {1,3,...,\bins}{
    \pgfmathparse{\i*1.0/\bins}
    \edef\ll{\pgfmathresult}
    \pgfmathparse{(\i+1)/\bins}
    \edef\rr{\pgfmathresult}
    \edef\temp{%
      \noexpand%
      \fill[group splitter] (rel axis cs:0,\ll) rectangle (rel axis cs:1,\rr);%
    }
    \temp
    %;
  }
}

